KaLM-Embedding-V2: Superior Training Techniques and Data Inspire A Versatile Embedding Model

Recent advancements in Large Language Models (LLMs)-based text embedding models primarily focus on data scaling or synthesis, yet limited exploration of training techniques and data quality, thereby constraining performance. In this work, we propose KaLM-Embedding-V2 from the Lychee-KaLM team, a series of versatile and compact embedding models, systematically incentivizing advanced embedding capability in LLMs by superior training techniques and high-quality data. For model architecture, we implement the models in a 0.5B compact size with simple mean-pooling to produce fixed-length embeddings and remove the causal attention mask to enable fully bidirectional representation learning. For training techniques, we propose a progressive multi-stage training pipeline: pre-training on weakly supervised large-scale datasets, fine-tuning with supervised high-quality datasets, and contrastive distillation with fine-grained soft signals, integrated with focal-style reweighting and online hard-negative mixing to emphasize difficult samples and enrich hard negatives, respectively. For training data, we curate over 20 categories for pre-training and 100 categories for fine-tuning and contrastive distillation to improve both performance and generalization, leveraging task-specific instructions, hard-negative mining, and example-based multi-class labeling to ensure high quality. Combining these techniques, our KaLM-Embedding-V2 series achieves state-of-the-art performance on the Massive Text Embedding Benchmark, outperforming models of comparable size and rivaling models 3--26x larger, setting a new standard for versatile and compact embedding models under 1B parameters. The code, data, and models are available at https://kalm-embedding.github.io/.

==> Table/focal_results.tex <==
\begin{table}[h]
  \renewcommand\arraystretch{1.05}
  \caption{Performance comparison \textit{w.r.t.} focusing parameter $\gamma$. $\gamma=0.5$ is the default setting, and $\gamma=0.0$ sets the weight of each sample to 1, indicating that reweighting has not been performed.}
  \tabcolsep=0.18cm
  \centering
  \footnotesize
  \begin{tabular}{l|cccccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}}   & \multicolumn{2}{c}{\textbf{MTEB (cmn, v1)}} & \multicolumn{2}{c}{\textbf{MTEB (eng, v1)}} & \multicolumn{2}{c}{\textbf{Avg}} \\
    \cline{2-7}
               & \textbf{MTK} & \textbf{MTY} & \textbf{MTK} & \textbf{MTY} & \textbf{MTK} & \textbf{MTY} \\
    \hline
    \textbf{KaLM-embedding-mini-instruct-V2~~($\gamma=0.0$)}   & 66.71 & 67.43 & 67.31 & 63.89 & 67.01 & 65.66 \\
    \textbf{KaLM-embedding-mini-instruct-V2~~($\gamma=0.5$)}   & \textbf{68.15} & \textbf{69.28} & \textbf{67.47} & \textbf{64.13} & \textbf{67.81} & \textbf{66.71} \\
    \bottomrule
  \end{tabular}
  
  \label{tab:focal_results}
\end{table}




==> Table/inference_latency.tex <==
\begin{wraptable}{r}{0.27\textwidth}
    \vspace{-0.43cm}
    \tiny
    \renewcommand{\arraystretch}{0.6} 
    \setlength{\tabcolsep}{0.27mm} 
  \centering
  \resizebox{0.27\textwidth}{!}{
  \begin{tabular}{l>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}}
    \toprule
    \textbf{Attn} & Retri. & STS \\
    \midrule
    BiAttn           & 1450s & 68s \\
    Causal           & 1448s & 70s \\
    \bottomrule
  \end{tabular}
  }
 \vspace{-0.2cm}
  \caption{Inference latency on MTEB (cmn, v1).}
  \label{tab:inference_latency}
  \vspace{-0.25cm}
\end{wraptable}

==> Table/model_soup.tex <==
\begin{wraptable}{r}{0.27\textwidth}
    \vspace{-0.43cm}
    \tiny
    \renewcommand{\arraystretch}{0.6} 
    \setlength{\tabcolsep}{0.27mm} 
  \centering
  \resizebox{0.27\textwidth}{!}{
  \begin{tabular}{l>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}}
    \toprule
    \textbf{Model} & MTK & MTY \\
    \midrule
    0           &  68.15 & 69.28 \\
    3           &  68.16 & 69.31 \\
    5           &  68.10 & 69.25 \\
    8           &  68.06 & 69.21 \\
    10           & 68.07 & 69.17 \\
    \bottomrule
  \end{tabular}
  }
 \vspace{-0.2cm}
  \caption{Results on MTEB (cmn, v1).}
  \label{tab:model_soup}
  \vspace{-0.25cm}
\end{wraptable}
